Revisiting Word Embeddings in the LLM Era

Large Language Models (LLMs) have recently shown remarkable advancement in various NLP tasks. As such, a popular trend has emerged lately where NLP researchers extract word/sentence/document embeddings from these large decoder-only models and use them for various inference tasks with promising results. However, it is still unclear whether the performance improvement of LLM-induced embeddings is merely because of scale or whether underlying embeddings they produce significantly differ from classical encoding models like Word2Vec, GloVe, Sentence-BERT (SBERT) or Universal Sentence Encoder (USE). This is the central question we investigate in the paper by systematically comparing classical decontextualized and contextualized word embeddings with the same for LLM-induced embeddings. Our results show that LLMs cluster semantically related words more tightly and perform better on analogy tasks in decontextualized settings. However, in contextualized settings, classical models like SimCSE often outperform LLMs in sentence-level similarity assessment tasks, highlighting their continued relevance for fine-grained semantics.

==> 4exp_dataset.tex <==
\section{Evaluation Framework}
To study the weather, the nine models (4-classical and 5-LLM) are able to differentially compare the pairs of words in contextualized and decontextualized settings. The settings are 
\subsection{Decontextualized Evaluation Setting}
\begin{itemize}[leftmargin=*,itemsep=0.2ex,partopsep=0ex,parsep=0ex]
    \item \textbf{\textit{Word-Pair Similarity Analysis}}: Given two distinct word embedding techniques (classical or LLM-based), we compare and analyze their cosine similarity distributions of pairs of 1) Semantically Related, 2) Morphologically Related, and 3) Unrelated words, where the distributions are derived from their word embedding vectors.
    
    \item \textbf{\textit{Word Analogy Task Analysis}}: For a given word analogy task of the form $a:b::c:d$ (``a is to b as c is to d''), we compare the accuracies of various embedding techniques using vector arithmetic in the latent vector space. %representations of $a$, $b$, and $c$ to make the result the nearest neighbor of $d$ are measured.
\end{itemize}

\subsection{Contextualized Evaluation Setting}
In our investigation of word embeddings in contextualized settings, we evaluated various models across nine different tasks. This list of tasks is not exhaustive but a subset of an exhaustive list. For the evaluation purpose, given a anchor word (a word which is either noun, verb, or adjective), we generate multiple sentences around the anchor words to put the word in some context. These sentence were then passed through models to extract both anchor word and sentence embeddings for evaluation. Since, there not existing dataset available, we generated synthetic samples by randomly selected 1,200 anchor words (nouns, verbs, or adjectives) from the WordNet dataset~\cite{fellbaum1998wordnet}. We then extracted the contextualized embeddings of these anchor words from the sentence embeddings across nine categories. These categories are:
\begin{itemize}[leftmargin=*,itemsep=0.5ex,partopsep=0ex,parsep=0ex]
    \item \textbf{\textit{Synonym Task}}: Given an anchor word, sentence $S_1$ is generated. Next, sentence $S_2$ is then created by replacing one word (other than the anchor word) place before the anchor word in $S_1$ with its \textit{synonym}. Finally, we compare the embeddings of the anchor word and the sentences.
    \item \textbf{\textit{Antonym Task}}: Given an anchor word, sentence $S_1$ is generated. Next, sentence $S_2$ is then created by replacing one word (other than the anchor word)  place before the anchor word in $S_1$ with its \textit{antonym}. Finally, we compare the embeddings of the anchor word and the sentences.
    \item \textbf{\textit{Negation Task}}: Given an anchor word, sentence $S_1$ is generated. Next, sentence $S_2$ is then created by adding negation before the anchor word in $S_1$. Finally, we compare the embeddings of the anchor word and the sentences.
    \item \textbf{\textit{Jumbling Task}}: Given an anchor word, sentence $S_1$ is generated. Next, five different sentences are created using $S_1$. Sentence $S_2$ is then created by shuffling words before the anchor word in sentence $S_1$. Sentence $S_3$ is created by randomly shuffling the complete sentence. Sentence $S_4$ and $S_5$ is created by exchanging one and two word around the anchor word respectively. Finally, we compare the embeddings of the anchor word and the sentences.
    \item \textbf{\textit{Paraphrasing Task}}: Given an anchor word, sentence $S_1$ is generated. Next, four more sentences are created as a paraphrase of sentence $S_1$ with anchor word common in all the sentences. Finally, we compare the embeddings of the anchor word and the sentences.
    \item \textbf{\textit{Active-Passive Task}}: Given an anchor word, sentence $S_1$ is generated in active voice. Next, sentence $S_2$ is created as a passive voice of sentence $S_1$ with anchor word common in both sentences. Finally, we compare the embeddings of the anchor word and the sentences.
    \item \textbf{\textit{Questionnaire Task}}: Given an anchor word, sentence $S_1$ is generated. Next, sentence $S_2$ is created as a questionnaire of sentence $S_1$ with anchor word common in both sentences. Finally, we compare the embeddings of the anchor word and the sentences.
    \item \textbf{\textit{Exclamation Task}}: Given an anchor word, sentence $S_1$ is generated. Next, sentence $S_2$ is created as a exclamatory of sentence $S_1$ with anchor word common in both sentences. Finally, we compare the embeddings of the anchor word and the sentences.
    \item \textbf{\textit{Polysemic Task}}: Given an anchor word, two sentences $S_1,S_2$ are generated, both containing the anchor word. Although the anchor word is the same, it is used in very different contexts in each sentence. Finally, we compare the embeddings of the anchor word and the sentences.
    
\end{itemize}



\section{Experiments Setup and Dataset}

\subsection{Embeddings}
This study employs a diverse range of embedding models from the past five years, categorized into two broad groups: Large Language Models (LLMs) with over 1B parameters and "Classical" models with under 1B parameters. The LLMs include: LLaMA2-7B and LLaMA3-8B (both dim $=4096$) from Meta AI \cite{touvron2023llama}, OpenAI's embedding model ADA-002 (dim $=1536$), and Google's PaLM2 embedding model Gecko-001 (dim $=768$)~\cite{anil2023palm}, OLMo-8B (dim $=4096$) ~\cite{olmo}, OpenELM-3B (dim $=3072$)~\cite{openelm} and, Mistral-8B (dim $=4096$)~\cite{mistral}. To more clearly see the differences between these models and older (``classical'') ones, Meta AI's LASER (dim $=1024$)~\cite{Artetxe_2019}, Universal Sentence Encoder (USE) (dim $=512$)~\cite{cer2018universal}, SimCSE (dim $=1024$) ~\cite{simcse} and SentenceBERT (SBERT) (dim $=384$)~\cite{reimers2019sentencebert} were also tested.\\
% We generated both decontextualized and contextualized embeddings from each model. For decontextualized embeddings, we fed only the input word into each model's tokenizer. For open-source models that tokenize the input as a single token, we used the final hidden state. For models employing sub-word tokenization, we averaged the final hidden states of each token, allowing the model to 'contextualize' sub-word tokens in hidden layers before combining them into a single representation.\\
% Additionally, we generated contextualized embeddings by feeding pairs of sentences from our proposed nine contextual tasks into each model. To extract in-context anchor word embeddings, we located the position of anchor words in both sentences and fetched their respective embeddings from the final hidden states. For sub-word tokenization, we averaged the embeddings from the hidden states to represent the word embedding.
% Due to API limitations, we excluded closed-source models like GPT-ADA-002 and PaLM-Gecko from the contextualized embedding analysis, as they do not allow fetching of tokenized embeddings. Similarly, we omitted classical models such as USE and LASER, which do not generate contextualized word embeddings.\\
% For decontextualized embeddings from closed-source models like ADA and PaLM-Gecko, we only had access to the final-layer activations for words. To ensure a uniform and fair evaluation across all models, we consistently used the last layer activations for our analyses. fair evaluation.
We generated both decontextualized and contextualized embeddings from each model. Decontextualized embeddings were created by inputting single words into each model's tokenizer. For models using single-token inputs, we utilized the final hidden state. In cases of sub-word tokenization, we averaged the final hidden states of each token. Contextualized embeddings were generated by inputting sentences from our proposed nine contextual tasks. We extracted in-context anchor word embeddings by locating the position of anchor words in the sentences and retrieving their respective embeddings from the final hidden states.\\
Due to API limitations, closed-source models like GPT-ADA-002 and PaLM-Gecko were excluded from the contextualized embedding analysis. Similarly, classical models such as USE and LASER, which do not generate contextualized word embeddings, were omitted from this part of the study. 
% For consistency across all models, we used the last layer activations for our analyses.
\subsection{Datasets Generation}
\subsection{Decontextualized Word Setting}
In an extension of the original analogy task set out by \citet{mikolov-etal-2013-linguistic}, \citet{gladkova-etal-2016-analogy} introduced Bigger Analogy Test Set (\textbf{BATS}), a larger set of related word pairs. This set is more comprehensive regarding the types of relations included and more forgiving in analogies with more than one correct answer~\cite{gladkova-etal-2016-analogy}. This dataset forms the basis for the evaluations performed in this paper.

\subsection{Contextualized Vs. Decontextualized Word Setting}
To analyze words in context, we generated sentence pairs across nine categories designed to explore word behavior in various scenarios: \textit{1) Synonym, 2) Antonym, 3) Negation, 4) Jumbling, 5) Paraphrase, 6) Active-passive, 7) Questionnaire, and 8) Exclamation}. Note that, the first four categories involve high word overlap between pairs.\\
We sampled 1200 unique words (called anchor words that are nouns, adjectives, and verbs) from WordNet~\cite{fellbaum1998wordnet} and used the \textit{Cluade-sonnet}~\cite{} model to generate sentences for each category based on these words. The system role for each category is detailed in the appendix~\ref{}.

For evaluation, we extracted three types of embeddings: 1) Decontextualized word embeddings: The anchor word embedding from each model. 2) Contextualized word embeddings: token-level anchor word embedding from the last hidden layer of each model and, 3) Sentence embeddings: The overall embedding for each generated sentence. 

This approach allows us to compare word representations in both contextualized and decontextualized settings across different models and sentence categories.










==> Tables/angle_table.tex <==
\begin{table*}[]
    \centering
    \ra{1.1}
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{r|cc|cc|cc|cc|cc|cc|cc|cc}
\toprule
 \multirow{2}{*}{Models} & \multicolumn{2}{c|}{Synonym} & \multicolumn{2}{c|}{Antonym} & \multicolumn{2}{c|}{Negation} & \multicolumn{2}{c|}{Polysemy} & \multicolumn{2}{c|}{Paraphrase} & \multicolumn{2}{c|}{Active-Passive} & \multicolumn{2}{c|}{Exclamatory} & \multicolumn{2}{c}{Questionnaire} \\
 \cmidrule{2-17}
 & Words & Sent. & Words & Sent. & Words & Sent. & Words & Sent. & Words & Sent. & Words & Sent. & Words & Sent. & Words & Sent. \\
% \multirow{2}{*}{Models} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\midrule
\midrule
SBert & 10.58 & 18.01 & 14.76 & 27.38 & 22.78 & 38.46 & 43.70 & 77.76 & 27.63 & 44.44 & 17.64 & 16.86 & 20.45 & 30.80 & 14.30 & 22.48 \\
SimCSE & 9.60 & 9.25 & 19.61 & 21.09 & 27.99 & 26.75 & 53.34 & 59.67 & 24.77 & 25.97 & 13.59 & 10.58 & 20.28 & 21.72 & 16.05 & 14.53 \\
\midrule
LLaMA3 & 14.07 & 12.31 & 19.27 & 17.06 & 27.87 & 21.72 & 64.15 & 55.04 & 40.09 & 27.87 & 43.86 & 26.36 & 35.51 & 28.24 & 28.36 & 23.22 \\
LLaMA2 & 13.59 & 12.84 & 20.61 & 16.86 & 27.13 & 22.78 & 59.40 & 49.91 & 44.19 & 27.38 & 47.55 & 27.25 & 36.68 & 28.24 & 27.75 & 22.18 \\
Mistral & 14.30 & 11.19 & 20.45 & 14.98 & 27.13 & 19.61 & 58.87 & 43.95 & 39.19 & 26.23 & 40.97 & 22.93 & 33.59 & 25.18 & 27.00 & 19.44 \\
OLMo & 16.26 & 13.59 & 21.41 & 18.74 & 29.19 & 24.49 & 64.85 & 57.45 & 45.09 & 31.90 & 46.21 & 30.34 & 40.18 & 32.11 & 32.01 & 24.49 \\
OpenELM & 8.51 & 8.51 & 14.07 & 9.94 & 17.64 & 13.09 & 49.53 & 30.34 & 26.36 & 20.93 & 27.38 & 13.83 & 22.48 & 16.46 & 16.86 & 10.89 \\
\bottomrule
\bottomrule
\end{tabular}
\end{adjustbox}
\label{cos_anlge}
\caption{Avg. of Angles (in degrees) b/w embeddings of Anchor words and Sentences (Sent.) in Contextualized Setting}
\end{table*}

==> prompting_box/exc_prompt.tex <==
\begin{boxI}\small
\label{exe_prompt}
\textit{\textbf{Paraphrase Pair Generation Prompting}}: \\\
\textbf{`System Prompt'}: \\
        Using the anchor word, create a sentence S1 that includes the anchor word. After generating S1, generate a sentence S2 which is an exclamatory sentence of sentence S1. It's crucial that S2 retains the anchor word in its original form. The anchor word must appear unchanged in both S1 and S2.\\
        
        Here is an example. For a given anchor word 'forum', the generated S1 and S2 sentences are:\\
        \{\\
        'sentence1': "The online forum attracted thousands of participants from various fields of expertise.",\\
        'sentence2': "What an incredible turnout the online forum attracted from thousands of participants across various fields of expertise!",\\
        'anchor\_word': 'forum'\\
        \}\\
        
        The output should be in the following json format: \\
        \{'sentence1: S1,\\
        'sentence2': S2, \\
        'anchor\_word': anchor\_word\\
        \}\\
        
        \textbf{User}: Here is the anchor word: {word}. Note that, the anchor word must appear unchanged in both S1 and S2.
    
\end{boxI}
